Shear measurement bias due to spatially varying spectral energy distributions in galaxies

Galaxy color gradients - i.e., spectral energy distributions that vary across the galaxy profile - will impact galaxy shape measurements when the modeled point spread function (PSF) corresponds to that for a galaxy with spatially uniform color. This paper describes the techniques and results of a study of the expected impact of galaxy color gradients on weak lensing measurements with the Large Synoptic Survey Telescope (LSST) when the PSF size depends on wavelength. The bias on cosmic shear measurements from color gradients is computed both for parametric bulge+disk galaxy simulations and for more realistic chromatic galaxy surface brightness profiles based on HST V- and I-band images in the AEGIS survey. For the parametric galaxies, and for the more realistic galaxies derived from AEGIS galaxies with sufficient SNR that color gradient bias can be isolated, the predicted multiplicative shear biases due to color gradients are found to be at least a factor of 2 below the LSST full-depth requirement on the total systematic uncertainty in the redshift-dependent shear calibration. The analysis code and data products are publicly available (https://github.com/sowmyakth/measure_cg_bias).

==> Makefile <==
# To make the document with the default settings:
# > make
#
# To make with a specific format:
# > make <format>
#
# To tar up a flat version of a specific format:
# > make <format> tar
#
# Alex Drlica-Wagner: https://github.com/LSSTDESC/start_paper/issues/new?body=@kadrlica

# Primary file names - avoid cookiecutter variables, to enable `make
# upgrade` to cleanly over-write this Makefile...
main=main
default=$(shell cat .metadata.json | grep 'default_format' | cut -d'"' -f4)
outname=$(notdir $(shell pwd))

ifeq ($(default), tex)
 style=tex
else
 style=${default}
endif

# LATEX environment variables
export TEXINPUTS:=./texmf/styles/:./tables/:
export BSTINPUTS:=./texmf/bib/:

# LaTeX journal class switcher flags
# apj=\def\flag{apj}
# apjl=\def
# mnras=\def\flag{mnras}

# Submission flags (these need some thought)
# arxiv=\def\flag{emulateapj}
# submit=${aastex}
# draft=\def\linenums{\linenumbers}

# Files to copy when making tarball
tardir=tmp
figdir=./figures
figures=$(figdir)/*.{png,jpg,pdf}
tabdir=./tables
tables=$(tabdir)/*.tex
styles=./texmf/styles/*.{sty,cls}
bibs=./texmf/bib/*.bst
source=$(main).{tex,bbl,bib} lsstdesc.bib acknowledgments.tex authors.tex contributions.tex

tarfiles=$(figures) $(tables) $(styles) $(bibs) $(source)

# Interpret `make` with no target as `make tex` (a latex Note).
# At present, if the default_format is anything other than
# [apj|apjl|mnras|prd|prl|emulateapj], a latex Note is made.
# In future, we could think of using `make` to eg run the ipynb
# notebook and make PDF from the output, but this has not been
# implemented yet.
all: export flag = \def\flag{${style}}
all: main copy

copy:
	cp ${main}.pdf ${outname}.pdf

touch:
	touch ${main}.tex

#http://journals.aas.org/authors/aastex/linux.html
#change the compiler call to allow a "." file
# 
main : authlist
	latexmk -g -pdf  \
	-pdflatex='openout_any=a pdflatex %O -interaction=nonstopmode "${flag}\input{%S}"'  \
	${main}
# 

tar : main
	mkdir -p ${tardir}
	cp ${tarfiles} ${tardir} | true
	cp ${outname}.pdf ${tardir}/${outname}.pdf
	cd ${tardir} && tar -czf ../${outname}.tar.gz . && cd ..
	rm -rf ${tardir}

authlist :
	pip install --upgrade mkauthlist
	mkauthlist -j ${style} -f -c "LSST Dark Energy Science Collaboration" \
		--cntrb contributions.tex authors.csv authors.tex

# http://stackoverflow.com/q/8028314/
TARGETS=apj apjl prd prl mnras tex aastex61 emulateapj
$(TARGETS): export style = $(@)
$(TARGETS): export flag = \def\flag{$(@)}
$(TARGETS):
	$(MAKE) -e main
	$(MAKE) -e copy
	$(MAKE) -e tar
# NB. the 'tex' target doesn't actually do anything in docswitch - make
# with no target compiles PDF out of main.tex using lsstdescnote.cls
# (which is to say, by default we assume you are writing an LSST
# DESC Note in latex format).

tidy:
	rm -f *.log *.aux *.out *.dvi *.synctex.gz *.fdb_latexmk *.fls
	rm -f *.bbl *.blg *Notes.bib ${main}.pdf

clean: tidy
	rm -f ${outname}.pdf ${outname}.tar.gz

# Update the tex styles etc:

baseurl=https://raw.githubusercontent.com/LSSTDESC/start_paper/master/%7B%7Bcookiecutter.folder_name%7D%7D

UPDATES=\
texmf/bib/apj.bst \
texmf/bib/mnras.bst \
texmf/styles/aas_macros.sty \
texmf/styles/aastex.cls \
texmf/styles/aastex61.cls \
texmf/styles/aps_macros.sty \
texmf/styles/docswitch.sty \
texmf/styles/emulateapj.cls \
texmf/styles/mnras.cls \
texmf/styles/lsstdescnote.cls \
texmf/styles/lsstdesc_macros.sty \
texmf/logos/desc-logo-small.png \
texmf/logos/desc-logo.png \
texmf/logos/header.png \
lsstdesc.bib \
.travis.yml \
figures/example.png

.PHONY: $(UPDATES)
$(UPDATES):
	curl -s -S -o $(@) ${baseurl}/$(@)
	@echo " "

update:
	@echo "\nOver-writing LaTeX style files with the latest versions: \n"
	@mkdir -p .logos figures texmf/styles texmf/bib
	$(MAKE) $(UPDATES)

# Get fresh copies of the templates etc, for reference:

TEMPLATES=\
acknowledgments.tex \
authors.csv \
main.ipynb \
main.md \
main.rst \
main.tex \
main.bib \
.metadata.json

.PHONY: $(TEMPLATES) templates
$(TEMPLATES):
	curl -s -S -o templates/$(@) ${baseurl}/$(@)
	@echo " "

templates:
	@echo "\nDownloading the latest versions of the template files, for reference: \n"
	@mkdir -p templates
	$(MAKE) $(TEMPLATES)
	$(MAKE) new
	ls -a templates/*

# Get a template copy of the latest Makefile, for reference:
.PHONY: new
new:
	@echo "\nDownloading the latest version of the Makefile, for reference: \n"
	@mkdir -p templates
	curl -s -S -o templates/Makefile ${baseurl}/Makefile
	@echo " "

# Over-write this Makefile with the latest version:
.PHONY: upgrade
upgrade:
	@echo "\nDownloading the latest version of the Makefile: \n"
	curl -s -S -o Makefile ${baseurl}/Makefile
	@echo "\nUpgrading version of mkauthlist: \n"
	pip install mkauthlist --upgrade --no-deps
	@echo "\nNow get the latest styles and templates with\n\n    make update\n    make templates\n"


==> authors.tex <==
% Author list file generated with: mkauthlist 1.2.2 
% mkauthlist -j tex -f -c LSST Dark Energy Science Collaboration --cntrb contributions.tex authors.csv authors.tex 

\author{Sowmya Kamath}
\affiliation{Department of Physics, Stanford University}
\affiliation{Kavli Institute for Particle Astrophysics and Cosmology (KIPAC)}

\author{Joshua Meyers}
\affiliation{Lawrence Livermore National Laboratory}

\author{Patricia Burchat}
\affiliation{Department of Physics, Stanford University}
\affiliation{Kavli Institute for Particle Astrophysics and Cosmology (KIPAC)}

\collaboration{(LSST Dark Energy Science Collaboration)}


==> contributions.tex <==
Author contributions are listed below. \\
alex: Initiated project, led development work. \\


==> latexmkrc <==
# This is an example latexmkrc file

# Set environment variables to search for tex inputs
# http://tex.stackexchange.com/a/50847/121099
$ENV{'TEXINPUTS'}='./texmf//:./tables/:' . $ENV{'TEXINPUTS'};
$ENV{'BSTINPUTS'}='./texmf/bib/:' . $ENV{'BSTINPUTS'};

# Set control tools
$pdf_mode = 1;
# You can change the \flag value here...
$pdflatex = 'openout_any=a pdflatex %O -interaction=nonstopmode "\def\flag{tex}\input{%S}"'

